PAGED: A Benchmark for Procedural Graphs Extraction from Documents

Automatic extraction of procedural graphs from documents creates a low-cost way for users to easily understand a complex procedure by skimming visual graphs. Despite the progress in recent studies, it remains unanswered: whether the existing studies have well solved this task (Q1) and whether the emerging large language models (LLMs) can bring new opportunities to this task (Q2). To this end, we propose a new benchmark PAGED, equipped with a large high-quality dataset and standard evaluations. It investigates five state-of-the-art baselines, revealing that they fail to extract optimal procedural graphs well because of their heavy reliance on hand-written rules and limited available data. We further involve three advanced LLMs in PAGED and enhance them with a novel self-refine strategy. The results point out the advantages of LLMs in identifying textual elements and their gaps in building logical structures. We hope PAGED can serve as a major landmark for automatic procedural graph extraction and the investigations in PAGED can offer insights into the research on logic reasoning among non-sequential elements.

==> Chapters/dataset-old.tex <==

% 0213
% \textcolor{red}{
% We use NLTK tool~\footnote{\url{https://www.nltk.org/}} to separate the documents in these datasets into multiple sentences, and then add marks to the boundaries between sentences as positive samples and insert marks into the interval of single sentence to construct negative samples. 
% }
% \textcolor{red}{
% In a standard procedural document, a single sentence~(``If he/she needs dishes, then choose the desired dishes and specify the taste.'') may convey the information of multiple procedural fragments~(\ding{192}, \ding{193} and \ding{195}). To achieve this, we proceed to combine separated fragments in each group into cohesive aggregations using another boundary identification model. This model is trained on collected data from~\citet{castelli2020techqa, zhang-etal-2020-reasoning, lyu2021goal} that contain more fine-grained separated segments. 
% }
% Additionally, to include actor information of actions, we add the prefix "For somebody:" before fragments related to the actor. For instance, we add "For customer:" before fragments containing actions executed by the customer. 

% At this point, we can obtain preliminary document by concatenating all the aggregations. 
% However, such generated documents lack fluency because each fragment is transferred using a hand-written template. Hence, we utilize ChatGPT for rephrasing the documents, leveraging its demonstrated near or even superior human-level performance in rephrasing task~\cite{chui2023chatgpt}. 
% Despite this, it is possible that some redundant actions from the generated documents that were retained during the Decomposition \& Transformation process will still be present after rephrasing, and ChatGPT will inevitably make some mistakes during rephrasing process. To remove redundant actions and fix rephrasing errors, we further refine the generated documents by hand-writing rules and making manual corrections, ultimately obtaining a total of 3394 high-quality documents. The statistics of the constructed dataset is shown in Table~\ref{dataset:statistics}. 
% See appendix~\ref{app:SurfaceSmoothing} for more details. 
\section{Dataset}

% V1
% Research for the procedural graph extraction from text heavily relies on large-scale and high-quality datasets, which consist of procedural graph and document pairs. 
% However, annotating the procedural graph based on corresponding document is a time-consuming and laborious task~\cite{maqbool2019comprehensive, bellan2020qualitative}. 
% Affected by the high annotation cost, existing datasets suffer from problems including small scale, incomplete procedural and factual knowledge representation and coarse-grained annotation. 

% Comparing to manually annotating procedural graphs based on procedural documents, our approach is less expensive and more efficient to implement with the help of automatic text generation technologies~\cite{zhang2023survey}, allowing for the construction of large-scale and high-quality dataset. 
% Moreover, such approach can better ensure the quality of the procedure graphs, as the existing procedure graphs are constructed by a large number of domain experts, which consume a lot of resources and have been validated by those experts. 

% V2
% Annotating the procedural graph based on corresponding document is challenging and laborious~\cite{maqbool2019comprehensive, bellan2020qualitative}. To construct high-quality dataset at a low cost, inspired by Data2Text task~\cite{lin2023survey}, we propose to supplement procedural documents for existing procedural graphs using available resources~\cite{dumas2018fundamentals}. 

% To promote optimal procedural graphs extraction, we use the Business Process Model and Notation (BPMN)~\cite{dijkman2011business} graph as the original procedural graph data for procedural documents supplementation. BPMN is the most commonly used type of procedural graph both in industry and academia~\cite{lopes2023assessing}. It is capable of complete procedural and factual knowledge representation~\cite{kocbek2015business, corradini2018guidelines} and is more complex and challenging compared to simple procedural graph containing only sequential actions, such as workflow~\cite{pal2021constructing, ren2023constructing}. This can help to evaluate whether existing studies can deal with the extraction of procedural graphs with higher complexity, in addition to the small-scale datasets that existing studies focus on. 
% involving a wide range of fields

% BPMN graphs consist of complete representations of various procedures, including plenty of complex branches and crucial constraints~\cite{corradini2018guidelines}, thus pose much more challenges than those containing only sequential actions, such as workflow~\cite{ren2023constructing}. 

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/DatasetConstruction.png}
%     \caption{The three-stage pipeline to supplement the procedural document based on the procedural graph.
%     }
%     \label{fig:DatasetConstruction}
% \end{figure*}

% V3
It is too costly to conduct an expert annotation of optimal procedural graphs for a large number of documents. As a remedy, we build our dataset upon a textbook~\cite{dumas2018fundamentals}, which has defined optimal procedural graphs covering the whole business process management lifecycle. In this way, the dataset construction turns into a data2text task --- generating a suitable document for a given procedural graph.
\subsection{Preliminary}
Figure~\ref{fig:task_b} presents an example of the optimal procedural graph. It describes the procedure of how a restaurant serves customers and involves two actors~(customer and restaurant). 
Each actor starts from the ``Start'' node, carries out actions following the logic in the graph, and ends at the ``End'' node. If the actions are performed sequentially, they are connected by the ``Sequence Flow''. Otherwise, there is an ``Inclusive Gateway'', ``Exclusive Gateway'' or ``Parallel Gateway'' indicating the following actions are non-sequential ones. Both the ``Inclusive Gateway''~(G-1) and ``Exclusive Gateway''~(G-3) mean that the following action is performed under the condition on the connected ``Condition Flow''. The difference is that there is one and only one condition after the ``Exclusive Gateway'' can be met, while this does not apply to the ``Inclusive Gateway''. The ``Parallel Gateway''~(G-5) represents that the following actions are performed in parallel. Note that, all gateways appear in pairs and the latter ones~(G-4, G-2, G-6) indicate the end of the non-sequential activities. Additionally, the ``Data Constraint'' and ``Action Constraint'' represent the necessary data~(C-1) and essential notices~(C-2) for actions connected by the ``Constraint Flow'', respectively.

% meaning the next action to be performed after the current condition is determined by specific conditions, 


% For each actor, starting from a ``Start'' notation, they execute the subsequent actions in the graph. Apart from simple sequential actions, the execution of non-sequential actions need to be represented by gateways. 
% % Gateway
% ``Exclusive Gateway''~(G-3) represents that the next action to be executed is determined by specific conditions. ``Inclusive Gateway''~(G-1) represents that one or more subsequent actions can be executed based on how many conditions are satisfied. 
% ``Parallel Gateway''~(G-5) represents the simultaneous execution of multiple actions. 
% % Constraint
% Additionally, ``Constraint'' represents the necessary data objects~(C-1) and essential notices~(C-2) for corresponding actions. 
% To integrate all elements and form a complete graph, ``Sequence Flow'' is used to connect different elements to show the progress of the procedure. Conditions used to determine executed non-sequential actions are represented by flows following exclusive and inclusive gateways. Furthermore, ``Constraint Flow'' links constraints with their corresponding actions. 

% 介绍图中的信息，主要是图例的定义和怎么看这个图
% \liang{xxxxxxxxxxxxx}
% As shown in Figure~\ref{fig:task_b}, the procedural graph starts from a 
\subsection{Dataset Construction}
With these high-quality procedural graphs, we then perform the dataset construction as a data2text task~\cite{lin2023survey}. Specifically, {we design a three-stage pipeline: 1) Decomposition \& Transformation that decomposes the graph into fragmented spans/sentences in natural language; 2) Grouping \& Ordering that logically organizes the procedural fragments; 3) Aggregating \& Smoothing that unifies the fragments into high-quality documents}. 

% Annotating procedural graph based on corresponding document is challenging and laborious~\cite{bellan2020qualitative}. To construct high-quality dataset at a low cost and promote optimal procedural graphs extraction, inspired by Data2Text task~\cite{lin2023survey}, we propose to build a dataset based on a business management textbook~\cite{dumas2018fundamentals}, which has summarized business processes into high-quality procedural graphs with complete sequential actions, non-sequential actions, and constraints. 

% Following ``easy to hard''~\cite{gao2023easy} strategy, we propose a three-stage pipeline to divide the document generation of an entire graph into manageable ones and solve them progressively, as shown in Figure~\ref{fig:DatasetConstruction}. 


% \liang{Check the comments here}
% 写作重点是要准确，不要写废话，只描述关键信息，对应图或者表中的例子，方法和实现步骤侧重描述我们针对本文任务做的特殊措施和改进
% 这部分写完了，改一版abstract出来，因为flow基本就可以定了，我们之后就算改了正文也可以只微调abstract了，控制20行左右


% 为了缩小直接从complex graph到length document之间的巨大gap，我们选择第一步将图分解为最小meaningful的单元，解释一些比较重要的定义，比如每个单元的第一个元素和最后一个元素不能是flow之类的，Note that 为了remain action之间的顺序或者约束？，哪些结点是重复遍历的，进一步为每个basic unit设计了template，这些template不一定是完整的句子，也可以是一些span，也费力去编写不同版本的template 只需要能够完整表达unit的意思就可以，我们把这些sentences/spans 统称为procedural fragments详细参见xxx

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/dataset/DatasetConstruction_1.png}
    \caption{Example of Decomposition \& Transformation.
    }
    \label{fig:Decomposition}
\end{figure}
\paragraph{Decomposition \& Transformation}
To narrow the huge gap between the complex graph and the length document, we first decompose the graph into minimal meaningful units. We define a vocabulary with nineteen units, each of which consists of actions, gateways or constraints connected by flow~(cf., Appx.~\ref{app:TriplesSplitting}). We also design nineteen hand-written templates for the vocabulary. Based on the unit vocabulary, we perform the breadth-first search strategy~\cite{10.1016/0004-3702(85)90084-0} over the graph, as shown in Figure~\ref{fig:Decomposition}. Note that, some actions may be repeatedly walked to preserve the sequential execution relation between adjacent actions in the graph. For example, ``Order drinks'' is walked twice, forming ``If need drinks, then order drinks.'' and ``order drinks, then specify the size.''. We then transfer the decomposed units into natural language spans/sentences based on the paired templates. We call these spans/sentences ``procedural fragments''. 

% Inspired by xxxx（我随便找了一篇Summarization of Diagrams in Documents，还有一些托福考试博客https://ielts-up.com/writing/task-1-diagram.html，你可以再让liao找一些更有说服力的参考文献）为了describe the detailed fragment in a logic way, 我们首先讲fragments进行分组。解释具体是怎么做的。每一组xxx（这个组具体代表了什么，一个subgoal，或者连贯执行的action之类的，这个你自己思考下）。
%由于xxx（需要排序的原因，因为你生成unit的时候肯定是按照一定顺序，为什么这个顺序还需要重新排一下，而且为什么可以只做组内排序）我们还进行了组内排序。解释具体是怎么做的，我们把order完的组叫做AAA（要不要起名字看你的选择）
% \begin{figure}[t]
%     \centering
%     \subfigure[Grouping]{\includegraphics[width=\linewidth]{figures/dataset/DatasetConstruction_2.png}
%     \vspace{-0.5cm}
%     \label{fig:Grouping}}

%     \vspace{-0.2cm}
%     \subfigure[Ordering]{\includegraphics[width=\linewidth]{figures/dataset/DatasetConstruction_3.png}\label{fig:Ordering}}

%     \caption{Example of Grouping \& Ordering.
%     }
%     \label{fig:Grouping_Ordering}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/dataset/DatasetConstruction_2.png}
    \caption{Example of Grouping \& Ordering.
    }
    \label{fig:Grouping_Ordering}
\end{figure}

\paragraph{Grouping \& Ordering}
When writing a procedural document, it is vital to provide information in a logical way, namely, describing the whole procedure sub-procedure by sub-procedure~\cite{futrelle1999summarization, futrelle2004handling}. Hence, we need to group the fragments into sub-procedures. We model this as a boundary identification task. Specifically, 
\textcolor{red}{
we train a boundary identification model using the WikiHow~\cite{bolotova2023wikihowqa} corpus that contains documents consist of numerous textual segments. We add separator token ``<SEP>'' between these segments to construct positive boundaries and insert separator tokens into the interval of the sentences within each segment to construct negative boundaries. A token classifier is then used to predict if each added separator token is a group boundary, allowing us to divide all fragments into different groups based on these predictions. 
}

% different groups using a boundary identification model. 
% Each group describes a sub-procedure of the whole procedure that is semantically coherent. 
% For example, we divide the customer's procedure before and after ``submit the order'' into two groups as shown in Figure~\ref{fig:Grouping_Ordering}. 
% We add a separator token ``<SEP>'' between every pair of adjacent fragments and employ a token classifier to predict the group boundaries of these fragments. 

\textcolor{red}{
After grouping, although the fragments in each group can together form a sub-procedure, the order that the algorithm traverses the graph not always aligns with how humans describe the actions in these fragments. 
For example, as shown in Figure~\ref{fig:Grouping_Ordering}, ``\ding{193}If need dishes, then choose the desired dishes'' should be immediately followed by ``\ding{195}choose the desired dishes, then specify the taste'', as only in this way, what the customer should do if meeting the condition ``need dishes'' can be continuously and coherently described. So we should order the fragments in Group1 to exchange the positions of fragment \ding{194} and \ding{195}. 
Therefore, we conduct fragments ordering within each group with a non-autoregressive ordering model~\cite{bin2023non}. 
We collect the data for model training from recent studies that provide off-the-shelf procedural documents consisting of sentences that describe a wide range of procedures~\cite{sakaguchi2021proscript, nandy2021question, bolotova2023wikihowqa}. We shuffle the sentences in the original documents and train the model to restore the order of these sentences. 
See appendix~\ref{app:NarrationAdjustment} for more details.}

% In a standard procedural document, 一些情况下，一个句子可以表述多个AAA. To achieve this, we xxx. 虽然到了这一步已经有了看似可以的document，但是由于模板的问题，这类document还不够流畅，所以我们利用Chatgpt, which has 在改写方面展现了接近甚至超越人类表现（citation），进行了润色。到这一步还没结束，因为一个好的procedural document应该是简洁而准确的---chatgpt并没有完全规避之前为了保证完整逻辑设置的重复节点的影响，文档仍存在一些冗余，同时由于chatgpt官方改写任务的特性，存在少量的错误修改。我们通过规则和人工校对进一步进行了xxx, 最终得到了高质量的document。
\paragraph{Aggregating \& Smoothing}
\textcolor{red}{
In a standard procedural document, a single sentence~(``If he/she needs dishes, then choose the desired dishes and specify the taste.'') may convey the information of multiple procedural fragments. To achieve this, we proceed to combine separated fragments in each group into cohesive aggregations using another boundary identification model. This model is trained on collected data from~\citet{castelli2020techqa, zhang-etal-2020-reasoning, lyu2021goal} that contain more fine-grained separated segments. 
}
Additionally, to include actor information of actions, we add the prefix "For somebody:" before fragments related to the actor. For instance, we add "For customer:" before fragments containing actions executed by the customer. 

At this point, we can obtain preliminary document by concatenating all the aggregations. 
However, such generated documents lack fluency because each fragment is transferred using a hand-written template. Hence, we utilize ChatGPT for rephrasing the documents, leveraging its demonstrated near or even superior human-level performance in rephrasing task~\cite{chui2023chatgpt}. 
Despite this, it is possible that some redundant actions from the generated documents that were retained during the Decomposition \& Transformation process will still be present after rephrasing, and ChatGPT will inevitably make some mistakes during rephrasing process. To remove redundant actions and fix rephrasing errors, we further refine the generated documents by hand-writing rules and making manual corrections, ultimately obtaining a total of 3394 high-quality documents. The statistics of the constructed dataset is shown in Table~\ref{dataset:statistics}. 
See appendix~\ref{app:SurfaceSmoothing} for more details. 


% \subsection{Basic Triple Splitting}
% \label{Splitting}
% To smooth out the gap between structured graph data and natural language text, we first split each procedural graph into basic triples according to the breadth first search~\cite{10.1016/0004-3702(85)90084-0} results of the graph, and then transfer them into natural language spans using hand-written templates. 
% For example, the triple ``(Inclusive gateway, need dishes, Choose the desired dishes)'' is transferred into ``If need dishes, then choose the desired dishes'' as shown in Figure~\ref{fig:DatasetConstruction}~(a). 
% See appendix~\ref{app:TriplesSplitting} for details. 

% \subsection{Narration Adjustment}
% \label{Narration Adjustment}
% % Due to the large amount of information contained in each procedure graph and the complex graph structure, simply concatenating all the transferred spans into single text may result in logical confusion and a lack of narrative hierarchy. To mimic the way humans describe the procedure graph, in which the entire graph is divided into different parts and described separately, we propose a three-step strategy to divide each graph into multiple groups and adjust the narrative order of the spans in each group. 

% % We adopt boundary identification methods and spans ordering models to adjust the narrative manner of the transferred spans for the entire graph. Through our elaborate adjustment, we are able to improve the semantic coherence of the generated text and the information consistency between the generated text and the original graph, as shown in Figure~\ref{}. 
% % For example, as shown in Figure~\ref{}, when encountering logical judgments, humans describe the situation of one branch first, and then go on to describe the remaining branches. 

% Simply concatenating all the transferred spans to form the document may result in confused expressions and the lack of coherence because inflexible templates are used. 
% To mimic the way humans describe the procedural graph, in which the entire graph is divided into different parts and described logically, we propose a ``Grouping-Ordering-Aggregating'' strategy to divide the spans of each graph into multiple groups, and adjust the narrative order and manner of the spans within each group. 
% See appendix~\ref{app:NarrationAdjustment} for details of adopted models and training corpus. 

% \paragraph{Grouping}
% % Instead of describing all the information in an entire graph continuously, humans divide the procedure graph into different parts and describe them one by one. 
% To improve the clarity and coherence of expressions for the generated documents, we use boundary identification model to divide the transferred spans into different groups. 
% For example, divide the customer's actions before and after ``submit the order'' into two groups as shown in Figure~\ref{fig:DatasetConstruction}~(b). 
% Inspired by \cite{narayan2017split}, we add a unique separator token ``<SEP>'' between every pair of adjacent spans and employ a token classifier to predict the group boundaries of each graph's spans. 
% % The predicted boundaries divide the spans into different groups for further transforming into fluent document. 

% \paragraph{Ordering}
% It is necessary to order the spans in each group because instead of describing the graph in the order that the algorithm traverses the graph in section~\ref{Splitting}, humans will adjust the narrative order of the information on the graph for clear and coherent expressions. 
% For example, as shown in Figure~\ref{fig:DatasetConstruction}~(c), ``If need dishes, then choose the desired dishes'' should be immediately followed by ``choose the desired dishes, then specify the taste'', as only in this way, what the customer should do if meeting the condition ``need dishes'' can be continuously and coherently described. 

% For effective spans ordering, we simultaneously utilize the non-autoregressive ordering model~\cite{bin2023non}, the autoregressive ordering model~\cite{calizzano2021ordering} and heuristic rules and compare their effectiveness later in section~\ref{Dataset Quality Evaluation} to determine the best one to use. 

% \paragraph{Aggregating}
% % To further improve the clarity of expression and narrative coherence of the generated document, we proceed with an aggregation process on the ordered spans. We combine separated spans into cohesive aggregations using with fine-grained boundary identification. By doing so, we can avoid confused expression of various procedural and factual knowledge through describing the generated document sentence by sentence. 

% After grouping and ordering, the spans in each group may still contain multifarious information, resulting in cumbersome expressions of each group. 
% Therefore, we proceed to combine separated spans in each group into cohesive aggregations using fine-grained boundary identification. 
% For example, as shown in Figure~\ref{fig:DatasetConstruction}~(d), we divide the spans of group~1 into three aggregations to coherently describe how the customer finds a seat, orders the dishes and drinks, and then submits the order. 
% Additionally, to include actor information in the original graphs, we prepend the text "For somebody:" before the spans corresponding to the actor, indicating that all subsequent actions in those spans are executed by that actor. For instance, we add "For customer:" before spans containing actions executed by the customer. 

% \subsection{Surface Smoothing}
% Due to the fact that the basic triples in the original graph are transferred by hand-written templates, the generated documents may appear mechanical for reading and are not as fluent as the text written by human. 
% As a result, as shown in Figure~\ref{fig:DatasetConstruction}~(e), we conduct rephrasing operation on the concatenation of the processed spans using large language model to smooth out the discontinuities between the spans and improve semantic coherence for the final generated document. We add the unique separator token ``<SEP>'' to indicate the group and aggregation boundaries of the spans for the rephrasing model, which can prompt the model to describe these spans coherently and clearly. Details are listed in the appendix~\ref{app:SurfaceSmoothing}. 


% eva
\subsection{Dataset Analysis}
% \section{Dataset Quality Evaluation}
\label{Dataset Quality Evaluation}

To verify the reliability of our constructed dataset, we conduct both automatic and human evaluations to evaluate: (1) whether the generated documents are consistent with the original graphs and (2) whether the generated documents read coherently and fluently. 
We further evaluate the generated documents that are directly rephrased by ChatGPT without grouping, ordering and aggregating process to demonstrate the effectiveness of our proposed three-stage pipeline. 

\input{tables/dataset_eva}
\input{tables/dataset_human}

% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/dataset/DatasetEva.png}
%         \caption{Automatic evaluation results of the generated procedural documents. "non-auto" refers to non-autoregressive ordering model, "auto" to autoregressive ordering model, and "heuristic" to heuristic rules.}
%         \label{fig:DatasetEva}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/dataset/DatasetHuman.png}
%         \caption{Human evaluation results of the generated procedural documents by different ordering approaches.}
%         \label{fig:DatasetHuman}
%     \end{minipage}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/dataset/DatasetEva.png}
%     \caption{Automatic evaluation results of the generated procedural documents. ``non-auto'' refers to non-autoregressive ordering model, ``auto'' refers to autoregressive ordering model and ``heuristic'' refers to heuristic rules.
%     }
%     \label{fig:DatasetEva}
% \end{figure}

\paragraph{Automatic Evaluation}
Following the evaluation strategies commonly used in Data2Text task~\cite{lin2023survey}, we adopt \textbf{FINE}~\cite{duvsek2020evaluating} and \textbf{ESA}~\cite{faille2021entity} to evaluate whether the generated documents fully cover the original graphs' information~(FINE-omission) and not contain redundant information~(FINE-hallucination), and maintain the entities and actions in the generated documents consistent with those in the original graphs~(ESA-entity \& action). 

As shown in Figure~\ref{fig:DatasetAuto}, evaluation results demonstrate that the generated documents processed by the full three-stage pipeline can achieve high consistency with the original graphs. The documents directly rephrased by ChatGPT fail to maintain high consistency as simply concatenate all fragments together can not present the information of the procedural graphs in a logic way, resulting in poor alignment between the generated documents and the original graphs. 

% As shown in Table~\ref{dataset_eva}, evaluation results demonstrate that both non-autoregressive and autoregressive ordering models can achieve high consistency with the original graphs. Heuristic rules fail to maintain high consistency as hand-written rules cannot cover various graph structures, resulting in incoherence of the generated documents.  


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/dataset/DatasetHuman.png}
%     \caption{Human evaluation results of the generated procedural documents by different ordering approaches.
%     }
%     \label{fig:DatasetHuman}
% \end{figure}

\paragraph{Human Evaluation}
\input{tables/dataset_statistics}

% To comprehensively evaluate the quality of the generated documents, we conduct human evaluation between the generated documents and the original graphs. 
We design five criteria to evaluate the generated documents through the rating of three experts, listed as follows:

\begin{itemize}
    \item \textbf{Understandable}: the generated document is capable of being understood. 
    \item \textbf{Adequacy}: the generated document fully covers all the information in the original graph. 
    \item \textbf{Hallucination}: the generated document does not contain any other information beyond the original graph. 
    \item \textbf{Coherence}: expressions of the generated document are coherent. 
    \item \textbf{Humanness}: the generated document reads like it was written by humans. 
\end{itemize}

\noindent
evaluators are required to rate each criterion on a scale of $1$ to $5$, with $5$ indicating that the generated document fully meets the requirements and $1$ indicating that it does not meet the requirements at all. 
We also report the ICC~(Intraclass Correlation Coefficient)~\cite{shrout1979intraclass} score to ensure the consistency between different evaluators and the evaluation effectiveness. Generally an ICC of $0.75$ or higher indicates that the evaluation is reliable~\cite{koo2016guideline}. 
% We report the average rating scores of different ordering approaches and the ICC scores in Table~\ref{dataset_human}. 

As shown in Table~\ref{fig:DatasetHuman}, 
the full three-stage pipeline can produce high-quality documents that are fluent and can achieve high equivalency with the original graphs. The generated documents directly rephrased by ChatGPT achieve lower scores that that processed by the full three-stage pipeline, because they fail to logically and coherently describe the procedural graphs, resulting in confusing expressions and incoherence of the generated documents. 
This indicates that it is necessary to group the fragments into sub-procedures, order the fragments within each group and combine separated fragments into cohesive aggregations, finally obtain high-quality documents. 

% We adopt the proposed three-stage pipeline and selected strategies to generate the procedural description text of corresponding raw procedure graph, and finally construct a total of 3394 samples, each with a pair of procedure graph and corresponding procedural description text. 
% The statistics of the dataset for our proposed benchmark \benchmark compared with the existing datasets for procedure graph extraction task is shown in Table~\ref{datasets}. 


==> Chapters/experiments-old.tex <==

\input{tables/exp_results}

\section{Experiments}
% To comprehensively evaluate the performance of existing studies, we select several representative models that perform best in current datasets from recent studies. 
% Meanwhile, we select the emerging large language models that perform well in various fields to explore whether these powerful large models can help to solve this task well. 

% It should be noticed that, due to the difficulty in generating procedure graph directly by the model, we use a dot language based textual representation~\cite{grohs2023large} in the form of ``NODE -> (condition) NODE'' as the equivalent representation of the graph structure. This can greatly facilitate our exploration of this task through the paradigm of text generation. 


We conduct systematic experiments to answer the two research questions: 
(1) \textit{whether the existing studies have well solved the automated extraction of procedural graphs from procedural documents}; (2) \textit{whether the emerging large language models can bring new opportunities to this task}. 

\subsection{Experimental Setup}

\subsubsection{Baselines}
% V1
% We select several representative models that perform best in current datasets to measure the performance of existing methods. And we also aim to explore the perform of the emerging large language models. 
% The selected baseline models can be divided into three categories. They are listed as follows:

% \begin{enumerate}[label=\Roman*., itemsep=3pt,topsep=3pt,parsep=0pt,leftmargin=16pt]
%     \item \textbf{Pipeline Based}:
%     \begin{enumerate}[itemsep=0pt,topsep=1pt,parsep=0pt,leftmargin=1pt]
%         \item[--] \textbf{Translation Like}: a machine translation like pipeline based on syntactic analysis, semantic analysis and transformation between source text and the target procedural graph~\cite{sonbol2023machine}. 
%         \item[--] \textbf{Beyond Rule}: a three-step pipeline to identify nodes of the procedural graphs with information extraction technologies and construct their relations by hand-written rules~\cite{neuberger2023beyond}. 
%     \end{enumerate}
    
%     \item \textbf{Elements Linking}:
%     \begin{enumerate}[itemsep=0pt,topsep=2pt,parsep=0pt,leftmargin=1pt]
%         \item[--] \textbf{Fact Types}: extracting elements on the procedural graphs based on an intermediate representation named fact types and linking them by hand-written rules~\cite{sholiq2022generating}. 
%         \item[--] \textbf{PET}: Conditional Random Fields based approach to support elements extraction and linking for the procedural graphs~\cite{bellan2022pet}. 
%         \item[--] \textbf{CIS}: using pre-trained language model to extract elements of the procedural graphs with in-context learning~\cite{bellan2022leveraging}. 
%     \end{enumerate}
    
%     \item \textbf{End to End}:
%     \begin{enumerate}[itemsep=0pt,topsep=1pt,parsep=0pt,leftmargin=1pt]
%         \item[--] \textbf{Flan-T5}: sequence-to-sequence language model trained on instruction data with a large scale number of downstream tasks~\cite{chung2022scaling}. 
%         \item[--] \textbf{Llama2}: generative text model that adapts to human preferences through supervised fine-tuning and reinforcement learning with human feedback~\cite{touvron2023llama}. 
%         \item[--] \textbf{ChatGPT}: a large language model with the ability to generate coherent responses through conversation~\cite{ouyang2022training}. 
%     \end{enumerate}
    
% \end{enumerate}

% V2
We select several state-of-the-art solutions to measure the performance of existing studies. And we also aim to explore the performance of the emerging large language models. 
The selected baseline models can be divided into three categories, listed as follows:

\paragraph{Pipeline Based}
(1) \textbf{Translation Like}: a machine translation like pipeline based on syntactic analysis, semantic analysis and transformation between source text and the target procedural graph~\cite{sonbol2023machine}. 
(2) \textbf{Beyond Rule}: a three-step pipeline to extract actions and gateways with information extraction technologies and construct the procedural graphs by hand-written rules~\cite{neuberger2023beyond}. 

\paragraph{Elements Linking}
(1) \textbf{Fact Types}: extract elements on the procedural graphs based on an intermediate representation named fact types and link them by hand-written rules~\cite{sholiq2022generating}. 
(2) \textbf{PET}: Conditional Random Fields based approach to support elements extraction and linking for the procedural graphs~\cite{bellan2022pet}. 
(3) \textbf{CIS}: use pre-trained language model to extract individual actions and conditions for their execution~\cite{bellan2022leveraging}. 

\paragraph{End to End}
(1) \textbf{Flan-T5}: sequence-to-sequence language model pre-trained with a large scale number of downstream tasks~\cite{chung2022scaling}. 
(2) \textbf{ChatGPT}: a large language model that can utilize in-context learning to facilitate procedural graphs extraction with designed instruction and a few examples~\cite{ouyang2022training}. 
(3) \textbf{Llama2}: a large language model capable of in-context learning and can be further fine-tuned on our dataset~\cite{touvron2023llama}. 


\subsubsection{Metric}
% Following current studies~\cite{Bellan2021ProcessEF, bellan2022pet, neuberger2023beyond}, we adopt standard F-1 score to evaluate the extracted procedural graphs in terms of nodes, edges, and actors. 
% For nodes evaluation, a node is considered successfully extracted only if the type and text of words of the node exactly match the type and text of words of the gold-standard label. After successfully matching the action nodes predicted by the model, we further consider the match of the actors for each action node. 
% For edge evaluation, an edge is considered successfully extracted only if the two nodes connected by the edge can exactly match the corresponding two nodes connected by the edge of the gold-standard label. 
% In addition, for edges connecting exclusive or inclusive gateways with other nodes, the conditions between extracted and gold-standard edges must also be matched. To avoid the disturbance of words' different morphology and tenses, we compare the stems of words of different texts and ignore the prepositions for soft comparison. 

% We adopt standard F-1 score to evaluate the extracted procedural graphs in terms of nodes, edges, and actors following current studies~\cite{bellan2022pet, neuberger2023beyond}. 
% A node is successfully extracted only if its type and text~(for actions and constraints) exactly match the gold-standard label. After matching the predicted action nodes, we then consider the match of actor for each action node. 
% An edge is successfully extracted only if its connected nodes and condition~(for edges connecting exclusive or inclusive gateways) exactly match those of the gold-standard label. 
% To avoid the disturbance of preposition words and words' morphology and tenses, we compare the stems of words of different texts. For example, ``submits the order'' is considered to be a successful match with ``submit the order''. 

The extraction of optimal procedural graphs requires not only identifying actions in the document, but more importantly: (1) using suitable gateways to represent the non-sequential execution of actions; (2) identifying vital constraints and actors of corresponding actions; (3) using flows to link all actions, gateways and constraints to form a complete procedural graph. 
Hence, we use BLEU~\cite{papineni2002bleu} metric to evaluate the model's accuracy in identifying actions, constraints, and actors. 
Then we use standard F1-score to evaluate the model's accuracy in using suitable gateways to represent non-sequential actions execution and correctly linking elements in procedural graphs using flows. 

Note that a flow is considered correctly extracted if its type and connected elements match those of the gold label. For a soft comparison, an element is considered matched with the gold label if its type matches the gold label and the BLEU score $\geq 0.5$~(gateways only require type match). 
For conditional flow, we compute the BLEU score between its condition and the gold label's condition if a condition flow in the gold label can be matched. 

\subsubsection{Implementation Details}
We divide our constructed dataset into three subsets: train set(1697 samples), validation set(543 samples), and test set(1154 samples), and evaluate the performance of all models uniformly on the test set. Pipeline Based and Elements Linking models do not require training data, except for PET trained on its own data. Therefore, we evaluate these models on our test set according to the original papers' setting. 
End to End models utilize our train set to fine-tune the model or construct examples for in-context learning, and use the validation set for model selection~\cite{raschka2018model}. 
To make good use of the capabilities of LLMs, we adopt the Chain-of-thought~(CoT)~\cite{wei2022chain} strategy to guide the inference process of extracting procedural graphs for the model, especially for the extraction of non-sequential actions. See Appx.~\ref{app:Experiments} for more details. 

\subsection{Results and Analysis}
% The performance of our proposed framework and baseline models are shown in Table~\ref{exp_results}. 
% Experimental results show the superiority of our proposed framework compared to other models, especially for the extraction of gateways. This demonstrates that our proposed framework can facilitate the model to better understand the complex branches in the documents and use correct gateways to represent them. 
% Additionally, we aim to answer the two research questions: 

\subsubsection{Performance of Existing Studies}
% V1
% Experimental results demonstrate that the existing studies are far from solving this task well. In fact, the existing studies neglects important inclusive gateways and the necessary factual knowledge in the procedural graphs, resulting in poor performance. 
% Additionally, we have the following observations:
% 1) Traditional Pipeline Based and Elements Linking methods generally perform worse than End to End methods. This is because the hand-written rules used by these methods can not cover various procedures in the real world, resulting in poor generalization. 
% 2) Due to the heavy reliance on syntax and semantic parsing, traditional methods are difficult to accurately extract action nodes from the procedural documents, as the complex expressions of the actions in the document are difficult to be fully extracted through parsing results and hand-written rules. 
% 3) The extraction of actors of corresponding action nodes is extremely challenging for traditional methods, as the expressions of actors in procedural documents are variable, making it difficult to extract the actors by rules. 
% 4) For Elements Linking baselines, CIS achieves better performance for action extraction with the help of pre-trained large model, but performs worse for exclusive gateway extraction than other two methods. This is because pre-trained large models are capable of understanding the surface semantic information of the text, but are not good at understand complex branches, which indicates that the combination of large models and insightful heuristic rules may be a way to solve this task. 

% V2
As shown in Table~\ref{exp_results}, 
experimental results demonstrate that existing studies are far from solving this task well as they perform poorly for the extraction of nearly all elements and neglect important gateways and constraints. 
Additionally, we have the following observations:
1) Traditional methods generally perform worse than End to End methods because hand-written rules used by them can not cover various procedures, resulting in poor generalization. 
2) Due to the heavy reliance on syntax and semantic parsing, traditional methods are difficult to accurately extract actions, constraints and actors from the procedural documents, as the complex expressions in documents are difficult to extract through parsing results and hand-written rules. 
3) For Elements Linking baselines, CIS achieves better performance for actions extraction with the help of large language model, but performs worse for gateways extraction than other two methods. This is because LLM is capable of understanding the surface semantic information of the text, but is not good at understand non-sequential execution of actions, which indicates that the combination of LLM and insightful heuristic rules may be a way to solve this task well. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figures/Method.png}
    \caption{The proposed two-system based self-refine framework. 
    }
    \label{fig:method}
\end{figure*}

\subsubsection{Performance of LLMs}
% V1
% Despite the fact that large language models can outperform traditional methods by a large margin, they still can not solve this task well, especially for the extraction of gateways. 
% Additionally, we have the following observations:
% 1) It should be noticed that although end to end methods perform well in extracting most nodes, they are difficult to surpass traditional methods for exclusive gateways extraction except fine-tuned Llama2 model. This indicates that large models adopted by end to end approaches have trouble understanding complex branches in the documents and determine correct gateways to represent them. 
% 2) For End to End baselines, it is difficult for them to distinguish exclusive and inclusive gateways correctly. Although fine-tuned on training data, Flan-T5 and Llama2 still perform worse than ChatGPT for the extraction of inclusive gateways. This is because the amount of training samples containing exclusive gateways is larger than that containing inclusive gateways,leading the model to learn harmful biases and cannot correctly determine the use of exclusive and inclusive gateways. 
% Our proposed framework successfully corrects these biases through external feedback with the two-system based self-refine strategy. 
% 3) Llama2 fine-tuned model can outperform traditional methods for node, edge, and actor extraction by a large margin, even surpassing ChatGPT. This indicates that large-scale and high-quality training data is crucial for exploring effective procedural graphs extraction model. Flan-T5 model is fine-tuned on the train set but performs worse than Llama2 fine-tuned model. This is probably because the causal language model architecture is more efficient to utilize in-context learning mechanism compared to the seq2seq language model architecture adopted by Flan-T5 model. 
% 4) The performance of edge and actor extraction largely depends on the accuracy of node extraction, because without accurately extracted nodes, it is impossible to construct correct edges between nodes and extract corresponding actors of the action nodes. Therefore, the challenge of this task mainly lies in the accurate extraction of the nodes, especially the gateways used to represent complex branches. 
% 5) Pre-trained large language models bring new opportunities for the extraction of procedural graphs containing both procedural and factual knowledge. But further improvements are needed to deal with the accurate extraction of complex branches and the construction of edges between the extracted nodes. 

% V2
Despite the fact that LLMs outperform traditional methods for identifying actions, constraints and actors by a large margin, they still struggle to represent non-sequential actions. 
Additionally, we have the following observations:
1) It should be noticed that although end to end methods perform well in extracting most elements, they are difficult to surpass traditional methods for gateways extraction except fine-tuned Llama2 model. This indicates that LLMs have trouble understanding non-sequential execution of actions in the documents and use correct gateways to represent them. 
2) For End to End baselines, it is difficult for them to distinguish exclusive and inclusive gateways correctly. Although fine-tuned on train set, Flan-T5 and Llama2 still perform worse than ChatGPT for the extraction of inclusive gateways. This is because the amount of training samples containing exclusive gateways is larger than that containing inclusive gateways,leading the model to learn harmful biases and cannot correctly determine the use of exclusive and inclusive gateways. 
3) Llama2 fine-tuned model can outperform traditional methods for the extraction of all elements, even surpassing ChatGPT. This indicates that large-scale and high-quality training data is crucial for exploring effective procedural graphs extraction model. Flan-T5 model is fine-tuned on the train set but performs worse than Llama2 fine-tuned model. This is probably because the causal language model architecture is more efficient to utilize in-context learning mechanism compared to the seq2seq architecture adopted by Flan-T5 model. 

\subsubsection{Improvement Strategies}
Through our detailed analysis of the extracted graphs of the LLMs, we find that understand the non-sequential execution of actions and use correct gateways to represent them is challenging for LLMs. 
To alleviate this defect, inspired by the ``dual process'' theories~\cite{evans2003two}, we design a two-system based self-refine framework to verify the extracted graphs of the model and provide external feedback to refine the model's extractions. 
As shown in Figure~\ref{fig:method}, we adopt the LLM as ``System1'' to extract the procedural graphs from the documents. Then we design two verifiers as ``System2'' to verify the correctness of the extracted graphs and provide feedback to the model for further refinement if needed. 


\paragraph{Condition Verifier}
% We design a ``condition verifier'' to verify the correctness of the exclusive and inclusive gateways extracted by the model. The models often fail to distinguish between these two types of gateways.

% After careful analysis, we find that the essential difference between exclusive and inclusive gateways lies in whether there exists conflict between the conditions of different branches. 
% For exclusive gateways, once the condition of one specific branch is satisfied, the conditions of other branches must not be satisfied, that is, all conditions of a single exclusive gateway are mutually ``exclusive''. 
% On the other hand, there exists no conflict between the conditions of a single inclusive gateway, that is, more than one conditions of the inclusive gateway can be satisfied at the same time. 

% Inspired by this, we design a simple and effective verifier to detect the conflict between the conditions of the branches and verify the correctness of corresponding gateways. 
% We adopt the off-the-shelf Natural Language Inference (NLI) model to measure the conflict between two conditions. If the conflict is detected for a inclusive gateway or no conflict is detected for an exclusive gateway, we will provide the feedback to the model. The model will further refine its predictions based on the provided feedback. 

The model often fails to distinguish between exclusive and inclusive gateways. 
After careful analysis, we find that the essential difference between exclusive and inclusive gateways lies in whether there exists conflict between the conditions need to be satisfied. 
Inspired by this, we design a simple and effective verifier to detect the conflict between the conditions of the extracted exclusive and inclusive gateways with off-the-shelf Natural Language Inference model, and provide the feedback to the model if: (1) a conflict is detected for inclusive gateways or (2) no conflict is detected for exclusive gateways. 
For example, the model extracts an exclusive gateway with conditions ``need dishes'' and ``need drinks'' that are not conflicted, and the verifier then provides feedback to the model for correcting the gateway type. 

\paragraph{Parallel Verifier}
% We design a ``parallel verifier'' to verify the correctness of the parallel branches predicted by the model and explore potential parallel branches that may have been missed by the model. 

We find that different actions can be executed in parallel only when the objects of these actions are different. On the contrary, if several actions are executed on a same object, they cannot be executed in parallel. 
Inspired by this, we design a verifier to verify the objects difference for parallel actions through semantic parsing. Additionally, we further explore the actions executed in sequence but on different objects, especially for those that meet the special syntactic pattern of ``same predicate with different objects'', which are capable of the potential for parallel execution and often neglected by the model. 
For example, two sequential actions ``prepare the meal'' and ``prepare the tableware'' have same predicate ``prepare'' and different objects, and the verifier then provides feedback to the model for extracting this potential parallel gateway. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/improve.png}
    \caption{Results of proposed improvement strategies and corresponding baseline models.
    }
    \label{fig:improve}
\end{figure}

% \input{tables/improvement}

\paragraph{Results}
% imporvement of strategies
As shown in Figure~\ref{fig:improve}, with the assistance of our proposed strategies, both ChatGPT and Llama2 achieve significant performance improvements for gateways extraction. This is because our proposed strategies help the model correctly understand the non-sequential actions in the documents and use correct gateways to represent them through external feedback provided by our designed verifiers. 
This indicates that the main challenge of utilizing LLM for optimal procedural graphs extraction lies in the comprehension and representation of non-sequential actions. 


% \paragraph{Self Refine}
% We provide feedback obtained from the two verifiers in ``System2'' to ``System1'' and promote the model in ``System1'' to refine the extracted graphs based on the feedback. 
% Due to space limitations, the specific templates used to generate the feedback are presented in the appendix. 

\subsection{Model Capabilities Analysis}
As shown in Figure~\ref{fig:Radar}, we divide the capabilities required for the extraction of optimal procedural graphs into seven dimensions and conduct comparison between several representative models to show their capabilities in different dimensions. 
We can see that compared with traditional methods, ChatGPT has greatly improved the capabilities in most dimensions, but there is no significant progress for gateway extraction. This indicates that even the powerful LLMs struggle to understand non-sequential actions in the documents. PET utilizes labeled training data to achieve improvement for action extraction compared to Translation Like model, but still performs poorly for gateway extraction. This is because the labeled data used by PET only contains individual action annotations and cannot help the model to learn represent non-sequential actions with correct gateways. Self-refined Llama2 alleviates these defects by fine-tuning on our constructed dataset and utilizing our proposed strategies. 
In general, existing solutions are still unable to accurately extract optimal procedural graphs from the documents, and the main challenge lies in the extraction of non-sequential actions. 

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{figures/Radar.png}
    \caption{Comparison of capabilities between several representative models. ``Gateway'' dimension represents the extraction of the three types of gateways. 
    }
    \label{fig:Radar}
\end{figure}

% advantages of various models and the challenges of this task

\subsection{Case Study}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Case.png}
    \caption{An example of the partial procedural graph extracted by our proposed framework from the document.
    }
    \label{fig:Case}
\end{figure}
As shown in Figure~\ref{fig:Case}, LLM with our proposed strategies can accurately extract complex non-sequential actions from the document, even in cases where different types of gateways are nested within each other. Through the feedback provided by our designed verifier, the model successfully understands that there exists no conflict between the two conditions "want some critic texture" and "enjoy the freedom lover", and correctly use the inclusive gateway to represent the non-sequential actions. 
Meanwhile, thanks to the strong semantic understanding ability of the LLM, it successfully identifies and extract the parallel actions hidden in the document. 



==> Chapters/intro-old.tex <==
% \section{Introduction}

% % Version1
% Procedures guide human and robots to achieve particular goals through describing and perceiving procedural knowledge in the world~\cite{miller1976natural, schank1977scripts, georgeff1986procedural}. Various forms of procedures, such as recipes~\cite{bien2020recipenlg}, manuals~\cite{liang2023knowing}, how-to guidelines~\cite{koupaee2018wikihow} etc., lead people to accomplish complex tasks. Automation technology of procedures can further assist the corporations in managing business process~\cite{dumas2018fundamentals}, answer user questions~\cite{nandy2021question}, support causal reasoning~\cite{zhang2020reasoning}, and even conduct in-depth planning through language model generation~\cite{qin2023tool, ruan2023tptu}. 

% The widespread application of procedure is mainly attributed to its structured representation~\cite{momouchi1980control, branavan2009reinforcement, addis2011unstructured}. 
% Current studies are devoted to revealing linear relationships between actions that make up the procedure. They naturally construct procedure as a sequence of actions and merely concern with pre- and post-conditions when reasoning the procedural knowledge~\cite{lyu2021goal, qasemi2022paco, wu2022learning, brahman2023plasma}. 
% However, the structures among actions are not always linear, especially when multiple actions exclude each other or time needs to be considerably saved~\cite{schrodt1990parallel, schrodt1994statistical, dumas2018fundamentals}. 
% Thus, these studies fail to represent actions' structure in more flexible and robust logical restrictions besides ordering them sequentially and thus overlook ''Put actions in parallel'' for procedures reasoning. 

% % Version2
% Procedures guide human and machines to achieve particular goals through describing and perceiving procedural knowledge in the world~\cite{miller1976natural, schank1977scripts, georgeff1986procedural}. To provide a more intuitive understanding for human and facilitate machine comprehension of complex procedures, they are formalized as structured representations~\cite{momouchi1980control, branavan2009reinforcement, addis2011unstructured}. 
% Among various types of representations, the graph representation of procedure, namely procedural graph, is most widely used due to its strong representational ability and ease of understanding by human and machines~\cite{friedrich2011process, zhang2012automatically, sonbol2023machine}. 

% However, obtaining such procedure graph is not easy. The construction of procedure graph is time consuming and cost intensive, which occupies most of the time and efforts spent in the research and application of procedural knowledge~\cite{herbst1999inductive, maqbool2019comprehensive, bellan2020qualitative}. To alleviate this problem, 
% procedure graph extraction technologies are proposed to automatically extract procedure graphs from various knowledge resources using information extraction strategies~\cite{friedrich2011process, honkisz2018concept, kretschmann2022design}. And the fact that procedural knowledge are often described in unstructured natural 
% language boosts the development of techniques to automatically extract procedure graphs from natural 
% language text~\cite{sholiq2022generating, neuberger2023beyond, sonbol2023machine}. 

% Procedural knowledge is generally described in unstructured natural language text~\citep{sonbol2023machine, ren2023constructing}.

% Although there is a large stock of texts containing procedural knowledge in the real world, the ablation of corresponding procedure graphs extracted from these texts largely hinders the development of procedure graphs extraction technologies due to their need of vast amount of data for exploring more effective models, resulting in poor performance and generalization of current studies~\cite{bellan2020qualitative, Bellan2021ProcessEF, zhu2023business}. Moreover, the ablation of a solid benchmark makes it difficult to compare existing approaches for procedure graph extraction and evaluate the performance of emerging natural language processing technologies such as large language models. 

% Version3
% Procedures guide human and machines to achieve particular goals through describing procedural knowledge in the world~\cite{miller1976natural, schank1977scripts, georgeff1986procedural}. To provide a more intuitive understanding for human and facilitate machine comprehension of complex procedures, they are formalized as procedural graphs~\cite{momouchi1980control, branavan2009reinforcement, addis2011unstructured}, which is capable of strong representational ability and ease of usability by human and machines~\cite{friedrich2011process, zhang2012automatically, sonbol2023machine}. Procedural graphs play an important role in many downstream tasks such as causal reasoning~\cite{zhang2020reasoning}, question answering~\cite{nandy2021question} and tool learning~\cite{qin2023tool, ruan2023tptu}. 


% Procedural documents (e.g. instruction books, user manuals, and cooking recipes), while are helpful to guide humans and machines to achieve particular goals~\citep{georgeff1986procedural}, entails massive efforts for humans to read and machines to comprehend~\cite{momouchi1980control, branavan2009reinforcement}. Representing procedural documents as structured procedural graphs thus has huge potential, as it offers an intuitive representation that is easy for humans to understand and promotes machine comprehension of procedures in downstream tasks, such as robotic systems automation~\cite{kovalchuk2021verifying}, procedures reasoning~\cite{zhou2022show}, and tool learning~\cite{qin2023tool, ruan2023tptu}. 


% Procedural graphs, though can intuitively represent the execution of actions for goal achievement~\cite{momouchi1980control, ren2023constructing}, suffer from the high cost of construction~\cite{herbst1999inductive, maqbool2019comprehensive}. 
% The automatic extraction of procedural graphs from procedural documents 
% % Procedural graphs extraction technology 
% thus has huge potential, as it would enable users to easily understand how to logically perform a goal~(e.g, how a restaurant serves the customers) by skimming visual graphs~(e.g., Figure~\ref{fig:task_b} instead of reading lengthy documents~(e.g., Figure~\ref{fig:task_a}). 


% the automatic production of procedural graphs~(Figure~\ref{fig:task_b}) from existing procedural documents~(Figure~\ref{fig:task_a}). 
% For example, extracting the procedural graph~from a document describing how a restaurant serves the customers. 

% However, obtaining optimal procedural graphs is not easy --- as shown in Figure~\ref{fig:task_b}, it requires representing not only sequential actions in the procedure~(e.g., \uppercase\expandafter{\romannumeral1}-4  $\rightarrow$ \uppercase\expandafter{\romannumeral1}-5), but also non-sequentially executed actions~(e.g., \uppercase\expandafter{\romannumeral1}-7.1 \& \uppercase\expandafter{\romannumeral1}-7.2]) and vital constraints for the actions~(e.g., C-2).  
% Off-the-shelf attempts only meet part of the requirements. For example, \citet{bellan2022pet, ren2023constructing} fail to represent ``customers can order only the dishes or drinks, or both''~(\uppercase\expandafter{\romannumeral1}-2.1 \& \uppercase\expandafter{\romannumeral1}-2.2) due to its inherent limitation for representing complex non-sequential actions. 
% Besides, current solutions only focus on hand-written rules~\cite{sholiq2022generating} or customized networks~\cite{bellan2022leveraging} on a small group of cherry-picked instances. This brings up the question of \textit{whether the existing studies have well solved the automated extraction of procedural graphs from procedural documents}. If the answer is ``no'', we are also interested in \textit{whether the emerging large language models~(LLMs) can bring new opportunities to this task}. 

% However, obtaining such procedural graphs is not easy. To extract procedural graphs from the documents, various approaches and datasets have been proposed to promote the transformation from procedural documents into procedural graphs~\citep{sholiq2022generating, neuberger2023beyond, sonbol2023machine}. 
% Nevertheless, current studies only conduct research on their individual small-scale datasets and the exploration of advanced natural language processing techniques is almost absent in these studies~\citep{bellan2020qualitative, Bellan2021ProcessEF}, so there exists two questions that urgently need to be answered: (1) whether the existing studies have well solved the task of procedural graphs extraction from documents; (2) if existing studies fail to achieve good performance, whether the emerging large language models can help to solve this task well. 

% But current studies fail to represent complete procedural knowledge and ignore important factual knowledge contained in the procedural documents, thus having trouble extracting complex procedural graphs. The ablation of solid dataset further hinders the development of procedural graphs extraction technologies due to their need of data resource for exploring more effective models~\citep{bellan2020qualitative}. 

% Furthermore, the ablation of large-scale and high-quality dataset greatly hinders the development of procedural graphs extraction technologies due to their need of data resource for exploring more effective models, resulting in poor performance and generalization of current studies~\cite{bellan2020qualitative, Bellan2021ProcessEF, zhu2023business}. And the ablation of a solid benchmark makes it difficult to compare existing individual works and evaluate the performance of emerging natural language processing technologies such as large language models~\citep{bellan2020qualitative, Bellan2021ProcessEF}. 

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/Task.png}
%     \caption{A toy example for the task of procedural graphs extraction from document. 
%     }
%     \label{fig:task}
%     \vspace*{-0.3cm}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \subfigure[procedural document]{\includegraphics[width=1\textwidth]{figures/Task_a.png}\label{fig:task_a}}

%     \vspace{-0.3cm}
%     \subfigure[extracted procedural graph]{\includegraphics[width=1\textwidth]{figures/Task_b.png}\label{fig:task_b}}
%     \vspace{-0.5cm}
    
%     \caption{A toy example for the task of extracting procedural graph (b) from the document (a).
%     }
%     \label{fig:task}
%     \vspace*{-0.3cm}
% \end{figure*}
% To answer the first question, we propose to construct a standard benchmark for the \underline{P}rocedur\underline{A}l \underline{G}raphs \underline{E}xtraction from \underline{D}ocuments~(\benchmark). As far as we know, there lack of large-scale datasets of document-graph pairs for training and evaluating optimal procedural graph extraction models~(cf., Table~\ref{datasets}). We want to equip \benchmark with the largest publicly available dataset. Although there exist plenty of procedural documents on the Internet, it is too costly to filter the low-quality ones and annotate optimal procedural graphs matching all requirements. Alternatively, we build the dataset based on a business management textbook~\cite{dumas2018fundamentals}, which has summarized business processes into high-quality procedural graphs with complete sequential actions, non-sequential actions, and constraints. Thus, constructing procedural document-graph pairs turns into assigning a suitable procedural document to a given procedural graph. We approach it via a three-stage pipeline --- we progressively transfer the structured information on the procedural graph into natural language text, adjust its narration and improve the coherence and naturalness, finally generating the suitable document. In this way, we develop a dataset with 3,394 high-quality procedural document-graph pairs that are about ten times than the previous largest datasets~\cite{ackermann2021data,qian2020approach}. According to the underlying structure of optimal procedural graphs, we introduce three types of metrics to evaluate six state-of-the-art methods~\cite{sonbol2023machine,neuberger2023beyond,sholiq2022generating}. 


% To answer these two questions, we propose a brand new benchmark named \benchmark for the task of \textbf{P}rocedur\textbf{A}l \textbf{G}raphs \textbf{E}xtraction from \textbf{D}ocuments. 
% We conduct a systematic study to reveal (\romannumeral1) the actual ability of existing studies and emerging large language models for procedural graphs extraction from documents; (\romannumeral2) the main challenges of this task. 
% As shown in Figure~\ref{fig:task}, an optimal procedural graph is capable of representing complex procedures with pre-defined notations. In addition to simple sequential actions, the non-sequentially executed actions~(called ``branches'')
% need to be represent with ``gateways''. 
% Parallel gateways~[F-5] represent the simultaneous execution of several actions. Exclusive gateways~[F-3] represent the next one action to be executed is determined by specific conditions on the edges. 
% Inclusive gateways~[F-1], ignored by existing studies, represent more than one action of the branches can be executed if multiple conditions are satisfied concurrently~\cite{dijkman2011business}. 
% Additionally, important constraints~[E-1 \& 2] about the action execution are also seldom considered by existing studies. 

% To support our systematic study, we propose a three-stage pipeline to construct a large-scale and high-quality dataset inspired by Data2Text task~\cite{gardent2017webnlg, lin2023survey}, which poses plenty of challenges for representing complex branches and crucial constraints as graphs. 
% Moreover, to alleviate the defects of current models, we propose a two-system based self-refine framework to facilitate the model to better understand complex branches and use correct gateways to represent them. 

% such as workflow~\cite{pal2021constructing, ren2023constructing}. 
% To ensure the quality of our constructed dataset, we propose a three-stage pipeline to generate the description text of each procedure graph. We first split the procedure graph into basic elements and adopt hand-written templates to transform them into natural language spans. Then we filter out uninformative spans and adjust the narrative order and manner of the filtered spans. Finally, we combine all the processed spans and rephrase them into smooth natural language text to obtain the final procedural description text for each original procedure graph. 

% Extensive experiments on our benchmark demonstrate that the extraction of procedural graphs from documents is a challenging task, and existing studies, even the powerful large language models are still far from solving this task well. Our proposed framework significantly advances the procedural graphs extraction by facilitating the model to better understand the complex branches in the procedures, but is still not enough to accurately extract the full procedural graphs from documents. 
% We hope our study on the proposed benchmark can promote the development of procedural graphs extraction from documents and facilitate the research and application of procedural graphs in the real world. 

% To further answer the second question, we investigate the performance of two on-trend LLMs~(ChatGPT~\cite{ouyang2022training} and Llama~\cite{touvron2023llama} and utilize a self-refine strategy to improve the ability of LLMs. In total, we evaluate nine methods in our \benchmark benchmark. Extensive experiments on our benchmark reveal that existing studies struggle to accurately extract sequential actions, non-sequential actions, and constraints from procedural documents. While large language models have shown significant improvement for sequential actions and constraints extraction compared to existing studies, they still face challenges with non-sequential actions extraction. Our detailed analysis of the results leads us to propose improvement strategies to help large language models better understand non-sequential actions and use correct gateways to represent them. 
% In summary, our contributions are listed as follows:
% % 这四个点都是只是描述了事实，没有突出亮点
% % 1. which后面主要解释我们这个东西可以回答两个提到的两个问题，我觉得你的某一版挺好的，你可以call back一下
% % 2. 数据集除了强调大，再说下，它的quality是通过我们的three-stage pipeline保证的，并且通过了自动和人工检验
% % 3. 这部分只强调，除了大模型之外问题的insight
% % 4. 这部分强调大模型的情况和未来的机遇
% % key point：不能泛泛而谈，得具体
% \begin{itemize}
%     \item We build a standard benchmark for procedural graphs extraction from documents, which help train and evaluate optimal procedural graph extraction models. 
%     \item We construct the biggest dataset with 3,394 high-quality procedural document-graph pairs that are about ten times than the previous largest datasets. 
%     \item We evaluate the performance of existing studies and the emerging large language models and reveal that they are still far from solving this task well. 
%     \item We point out that the main challenges of optimal procedural graphs extraction lie in the non-sequential actions extraction. 
% \end{itemize}

% \textcolor{red}{

% }


% Writing reference
% We develop a suite of three progressively harder tasks built around this contestto test how well AI models “understand’ humoracross vision and language: 1) matching jokes to cartoons, 2) identifying a winning caption, and 3)generating an explanation of why an image/captioncombination is funny. 



==> Chapters/method.tex <==
\section{Method}
% Accurately extracting procedural graphs requires the model to not only recognize the actions described in the document, but more importantly, to understand the logical branches and use correct gateways to represent them, which is challenging and crucial for the representation of complex procedures. 

% Traditional methods have trouble extracting accurate procedure graphs that contain complex logical judgments, because hand-written rules are difficult to cover various logical judgments and the potential of neural network models is hard to be fully explored due to limited data resource. 

% The emergence of large models provides a new opportunity to extract procedure graphs with complex logical judgments. However, current large models are still struggle to select correct gateways to represent conditional branches and recognize parallel branches contained in the procedural description text.

% Traditional methods have trouble extracting procedural graphs containing complex logical branches. And the emerging large models are also struggle to understand complex logical branches and determine correct gateways to represent them. 
% To alleviate these shortcomings, we propose a framework to enhance the model's extraction of procedural graphs containing complex logical branches. Inspired by the ``dual process'' theories~\citep{evans2003two}, we design a two-system based self-refine framework to verify the extracted graphs of the model and provide external feedback to refine the model's predictions. 

Understand the complex branches in the procedures and use correct gateways to represent them is challenging for traditional methods and even the large language models. 
To alleviate this defect, inspired by the ``dual process'' theories~\citep{evans2003two}, we design a two-system based self-refine framework to verify the extracted graphs of the model and provide external feedback to refine the model's extractions. 

\subsection{Overview of Proposed Framework}
As shown in Figure~\ref{fig:method}, we adopt the large language model~(LLM) as ``System1'' to extract the procedural graphs from the documents. Then we design two verifiers as ``System2'' to verify the correctness of the extracted graphs and provide feedback to the model for further refinement if needed. 
Because each procedural graph is composed of nodes~(e.g., actions and gateways) and edges~(e.g., sequential edges used to connect different actions and gateways), 
we use a dot language~\citep{gansner2006drawing} based graph representation in the form of ``Node -> (condition) Node'' to represent extracted graphs. 
For simplicity, we use ``XOR'', ``OR'' and ``AND'' as abbreviations for exclusive, inclusive and parallel gateways respectively. And we use numbers as suffixes to distinguish multiple gateways of the same type on the graph. 
Additionally, we require the model to output the actors of corresponding extracted actions for actors predictions. See appendix~\ref{app:ProposedMethod} for more details. 


\paragraph{Condition Verifier}
% We design a ``condition verifier'' to verify the correctness of the exclusive and inclusive gateways extracted by the model. The models often fail to distinguish between these two types of gateways.

% After careful analysis, we find that the essential difference between exclusive and inclusive gateways lies in whether there exists conflict between the conditions of different branches. 
% For exclusive gateways, once the condition of one specific branch is satisfied, the conditions of other branches must not be satisfied, that is, all conditions of a single exclusive gateway are mutually ``exclusive''. 
% On the other hand, there exists no conflict between the conditions of a single inclusive gateway, that is, more than one conditions of the inclusive gateway can be satisfied at the same time. 

% Inspired by this, we design a simple and effective verifier to detect the conflict between the conditions of the branches and verify the correctness of corresponding gateways. 
% We adopt the off-the-shelf Natural Language Inference (NLI) model to measure the conflict between two conditions. If the conflict is detected for a inclusive gateway or no conflict is detected for an exclusive gateway, we will provide the feedback to the model. The model will further refine its predictions based on the provided feedback. 


The model often fails to distinguish between exclusive and inclusive gateways. 
After careful analysis, we find that the essential difference between exclusive and inclusive gateways lies in whether there exists conflict between the conditions need to be satisfied. 
Inspired by this, we design a simple and effective verifier to detect the conflict between the conditions of the extracted exclusive and inclusive gateways with off-the-shelf Natural Language Inference model, and provide the feedback to the model if: (1) a conflict is detected for inclusive gateways or (2) no conflict is detected for exclusive gateways. 
For example, the model extracts an exclusive gateway with conditions ``need dishes'' and ``need drinks'' that are not conflicted, and the verifier then provides feedback to the model for correcting the gateway type. 

\paragraph{Parallel Verifier}
% We design a ``parallel verifier'' to verify the correctness of the parallel branches predicted by the model and explore potential parallel branches that may have been missed by the model. 

We find that different actions can be executed in parallel only when the objects of these actions are different. On the contrary, if several actions are executed on a same object, they cannot be executed in parallel. 
Inspired by this, we design a verifier to verify the objects difference for parallel actions through semantic parsing. Additionally, we further explore the actions executed in sequence but on different objects, especially for those that meet the special syntactic pattern of ``same predicate with different objects'', which are capable of the potential for parallel execution and often neglected by the model. 
For example, two sequential actions ``prepare the meal'' and ``prepare the tableware'' have same predicate ``prepare'' and different objects, and the verifier then provides feedback to the model for extracting this potential parallel gateway. 

% \paragraph{Self Refine}
% We provide feedback obtained from the two verifiers in ``System2'' to ``System1'' and promote the model in ``System1'' to refine the extracted graphs based on the feedback. 
% Due to space limitations, the specific templates used to generate the feedback are presented in the appendix. 



==> Chapters/related-old.tex <==
% statistics
\input{tables/datasets}

\section{Related Work}
\paragraph{Procedural Graph Extraction} 
% 论述逻辑是跟着intro走，大部分工作只能表达sequential actions， xxx补充了constraint， xxx干了啥，但是没有meet all requirements的。 Besides，这些工作largely是规则，有一篇是定制的神经网路，是否真的有用存疑。
Existing studies only meet part of the requirements for optimal procedural graph extraction. 
Earlier studies mainly focus on extracting sequential actions~\cite{pal2021constructing, lopez2021declarative, ren2023constructing}. 
While \citet{epure2015automatic, honkisz2018concept, bellan2022pet} explore non-sequential actions, they do not cover scenarios like \uppercase\expandafter{\romannumeral1}-2.1 \& \uppercase\expandafter{\romannumeral1}-2.2 in Figure~\ref{fig:task_b}. \citet{friedrich2011process} aids in data constraint extraction but overlooks action constraints. 
Besides, current studies heavily rely on hand-written rules and templates~\cite{epure2015automatic, honkisz2018concept}, resulting in poor generalization. \citet{bellan2022pet} trains a neural network model but only learns 45 samples, whose effectiveness remains questionable. 
% \liang{xxxxxxxxxxxxxxxx}% 需要补充结论，这些工作是否真的可以解决这个任务仍然存疑，所以我们要建立benchmark来探究下
% Therefore, we propose our benchmark to reveal the performance 
Hence, we propose to construct a standard benchmark to reveal the performance of existing studies and highlight the challenges for the extraction of optimal procedural graphs. 

% refers to the automatic extraction of procedural graphs from procedural documents~\cite{bellan2020qualitative}. 
% also Earlier works largely focus on designing more and more elaborate hand-written rules and templates~\cite{friedrich2011process, epure2015automatic, honkisz2018concept}. For example, \citet{epure2015automatic}. 
% Note that, the procedural graphs in this paper are different from graphs defined in \citet{kiddon2015mise,liang2023knowing}, which aim to improve the 


% Procedural graph extraction technologies are proposed to automatically extract the procedural graphs from natural language text~\cite{bellan2020qualitative}. Some studies try to extract procedural graphs through syntactic and semantic analysis of the text~\cite{friedrich2011process, epure2015automatic, honkisz2018concept}, but these studies heavily rely on hand-written rules and templates and are difficult to achieve good performance due to poor generalization ability. 
% Other studies adopt artificial neural network to improve the model performance~\cite{pal2021constructing, bellan2022pet, ren2023constructing}. However, these studies fail to achieve good performance due to limited data resource and the lack of representational ability for complex non-sequential actions and constraints. Therefore, we propose a solid benchmark and a two-system based self-refine framework to facilitate the development of optimal procedural graphs extraction. 


% \subsection{Actions Inference}
% Earlier studies exploited how to induce procedures from structured data, such as process model mining from event-log~\cite{agrawal1998mining, van2004workflow, van2012process}. However, the fact that large amounts of data describing procedures is stored as unstructured information has posed a more severe challenge for extracting procedural knowledge from unstructured data (e.g. natural language procedural description)~\cite{bellan2020qualitative, bellan2022pet, grohs2023large}. 
% Moreover, the emergence of large language models with powerful planning capabilities nowadays attracts researchers to explore the generation of structured procedures from scratch~\cite{brahman2023plasma, yuan2023distilling, qin2023tool}. 
% Although these studies promote procedural knowledge to be applied in real-world tasks, their inference strategy of ordering actions sequentially hinders more complex application that requires parallel execution for non-linear actions ordering. 

% \subsection{Actions Ordering}
% To construct inferred actions into structured representation, reasoning about relationships between actions is needed to determine their execution order. Current studies are devoted to handle the pre- and post-conditions for actions ordering~\cite{kwon2020modeling, wu2022learning, qasemi2022paco}. However, such inference strategy can only determine the sequence of linear execution of actions, which does not allow for the discovery of parallel execution patterns between actions. 
% Other studies directly model the partial order relationship between actions in end-to-end manners~\cite{sakaguchi2021proscript, brahman2023plasma, grohs2023large}. However, these approaches fail to proactively discover the potential parallel relationships between actions, resulting in poor performance for parallel orders reasoning. 

% \subsection{Procedures Representation}
% Existing studies formalize procedural knowledge in two types of structured representations, namely, action centered and entity centered. Action centered representations take action verbs as the core to represent ''what steps a procedure contain'' and show arguments and conditions modifying corresponding actions~\cite{zhang2012automatically, kiddon2015mise, zhou2022show}. Entity centered representations focus on the relationships between entities and the changes in entity status during the procedures~\cite{gupta2019tracking, gupta2019effective, li2023understand}. However, these studies treat actions and entities in procedures discretely and make it difficult to reach a unified representation, thereby hindering supporting a diverse range of applications that requires both declarative and procedural knowledge. In fact, procedures can be seen as a sequence of actions to reach a certain goal state from a certain starting state, according to~\cite{pareti2018representation}. Therefore, we can simultaneously model declarative and procedural knowledge through a unified representation for procedures reasoning. 


% V1
% To advance the development of automatic procedural graphs extraction from documents, many datasets have been proposed by existing studies. 
% The first dataset with 47 procedural graph and document pairs was presented by \cite{friedrich2011process}. Subsequently, \cite{epure2015automatic} and \cite{ferreira2017semi} proposed their own datasets but are not publicly available. Later, \cite{mendling2019natural} proposed a dataset with 103 samples but containing only sequential actions. A dataset with 360 samples was presented by \cite{qian2020approach}, which contains no branches and only includes sentence-level annotation. 
% \cite{ren2023constructing} constructs a procedural graph dataset but only focuses on sequential actions. 
% The datasets proposed by \cite{quishpi2020extracting, ackermann2021data, lopez2021declarative, bellan2022pet} are subsets of datasets that have been proposed in earlier studies mentioned above. 
% Consequently, as shown in Table~\ref{datasets}, despite the fact that many datasets have been proposed thus far, they fail to cover the research of optimal procedural graphs. And the lack of a solid benchmark for equitable comparison makes it difficult to advance the development of more effective models. 
% Therefore, we propose our benchmark to reveal the limitations of existing studies and highlight the challenges for the extraction of procedural graphs from documents, which can help to promote future studies in this field. 


% Table~\ref{datasets} displays the statistics of our constructed dataset in comparison to the existing datasets. 
% Due to the problems including small scale, incomplete procedural and factual knowledge representation, and coarse-grained annotation, current studies fail to explore effective models that necessitate large amounts of high-quality data. 
% We propose our benchmark to reveal the limitations of existing studies and highlight the challenges for the task of procedural graphs extraction from text, which can help to promote future studies in this field. 

% Enlarging the amount of available data is a significant challenge that current studies must overcome, because large-scale and high-quality datasets are crucial for the exploration of optimal procedural graphs extraction but are costly to obtain~\cite{bellan2020qualitative}. 
% As shown in Table~\ref{datasets}, 
% the first available dataset was presented by \cite{friedrich2011process} but contains only 47 samples. 
% Subsequently, \cite{epure2015automatic} and \cite{ferreira2017semi} proposed their datasets but are not publicly available. 
% Later, \cite{mendling2019natural}, \cite{qian2020approach} and \cite{ren2023constructing} proposed their own datasets with 103, 360 and 283 samples respectively. However, these datasets only contain sequential actions and can hardly be seen as representative of the variety of optimal procedural graphs. 
% Other datasets proposed by \cite{quishpi2020extracting, ackermann2021data, lopez2021declarative, bellan2022pet} are subsets of the above datasets. 

% V2 
\paragraph{Datasets}
% 参考 acl findings related work dataset的写法，论述重点是表格里面的两点数据，比如number，比如对号叉号，总结着说，参考下托福或者雅思表格题是怎么总结的

As shown in Table~\ref{datasets}, current datasets consist of a small group of cherry-picked instances. 
Some datasets are not publicly available~\cite{epure2015automatic, ferreira2017semi}. 
Some datasets only focus on sentence-level actions extraction, lacking both sequential and non-sequential actions~\cite{quishpi2020extracting, qian2020approach, ackermann2021data}. While other studies contain sequential actions~\citet{friedrich2011process, mendling2019natural, lopez2021declarative, bellan2022pet, liang2023knowing, ren2023constructing}, they do not cover all types of non-sequential actions. Moreover, almost all existing datasets ignore important constraints related to the actions in procedural graphs. To this end, we construct a new procedural document-graph dataset that is nearly ten times larger than the previous largest datasets~\cite{ackermann2021data,qian2020approach}. Each sample consists of a high-quality procedural document and its procedural graphs with complete sequential actions, non-sequential actions, and constraints.

% which is nearly ten times larger than the previous largest datasets~\cite{ackermann2021data,qian2020approach}. 


% To fill the blank of large-scale datasets for training and evaluating optimal procedural graph extraction model, we build a dataset based on a business management textbook~\cite{dumas2018fundamentals} that has gathered high-quality procedural graphs with complete sequential actions, non-sequential actions, and constraints. 
% 通过总结，需要把表格中的所有论文都引一遍，不能漏，一共11个

\paragraph{Data2Text}
% 需要突出下procedural的不同，为啥我们要用三阶段来做，不能只说因为他们不没做我们做了
Data2Text task aims at transferring structured data such as graphs into natural language text~\cite{duong2023learning, lin2023survey}. 
Current studies~\cite{su2021few, kasner2022neural} only focus on the transformation of factual knowledge --- knowledge about features of things, making it difficult to deal with procedural knowledge --- execution of sequential and non-sequential actions in the procedural graphs. 
\liang{Moreover, current studies can only manage small pieces of data~\cite{ye2019variational, fu2020partially}, but handling procedural graphs necessitates additional steps to integrate individual actions and constraints into a unified document. 
Hence, we propose a three-stage pipeline to transfer individual actions and constraints into natural language spans and seamlessly incorporate them into coherent document, imitating how humans describe procedural graphs}. 

% Some studies aim at transferring single structured data into natural language span~\cite{ye2019variational, fu2020partially}, but these studies are difficult to deal with numerous elements on the procedural graphs and transfer an entire procedural graph into document. 
% Other studies are capable of simultaneously integrating multiple structured data into text spans~\cite{moryossef2019step, ferreira2019neural, su2021few, kasner2022neural}. However, these studies only focus on factual knowledge --- knowledge about features of things, making it difficult to deal with the actions and gateways involved in the procedural graphs. To address these defects, we propose a three-stage pipeline to generate procedural document for the existing procedural graphs. 


\paragraph{Large Language Models}
The emerging LLMs have shown competitive results in a wide range of tasks~\cite{zhao2023survey, min2023recent}. 
However, the application of LLMs for procedural graph extraction nearly remains unexplored. 
The only exception is \citet{bellan2022leveraging}, who just makes a shallow attempt to extract sequential actions and partial non-sequential actions with LLM, \liang{and totally ignore constraints}. 
\liang{LLMs can utilize in-context learning~\cite{dong2022survey} strategy to solve many complex tasks, which remain unexplored on our task.} We then conduct a systematic study to reveal the opportunities brought by LLMs and find that they still struggle to extract non-sequential actions. 

% \liang{The only exception is \citet{bellan2022leveraging}, who employ large language models to extract individual actions from documents but still depend on hand-written rules to construct the procedural graphs. 
% Therefore, we investigate the performance of two on-trend LLMs~(ChatGPT~\cite{ouyang2022training} and Llama~\cite{touvron2023llama} to explore the opportunities brought by large language models.} 


% llms还有在xxx方面又能力，也需要在我们任务上研究下
% 我们研究了也提出了self-refine的策略，发现了潜力，也发现了不足


==> tables/ablation.tex <==
\begin{table}[t]
\caption{Experimental results of ablation study. ``w/o Condition Verifier'' and ``w/o Parallel Verifier'' mean not providing feedback from condition verifier and parallel verifier to the model respectively.}
\label{ablation}
\centering
\scalebox{0.7}{
\begin{tabular}{l|cccc}
\hline
\multicolumn{1}{c|}{Model} & XOR     & OR      & AND     & NodeTotal \\ \hline
Self-refine ChatGPT              & 0.5085  & 0.2487  & 0.4081  & 0.6335      \\
- w/o Condition Verifier     & -0.0425 & -0.0589 & -0.0038 & -0.0007     \\
- w/o Parallel Verifier      & -0.0072 & 0.0011  & -0.0237 & -0.0026     \\ \hline
Self-refine Llama2               & 0.5814  & 0.2983  & 0.4511  & 0.6964      \\
- w/o Condition Verifier     & -0.0356 & -0.209  & -0.0017 & -0.0102     \\
- w/o Parallel Verifier      & -0.0024 & -0.0042 & -0.0492 & -0.0080    
\end{tabular}
}
\end{table}



==> tables/dataset_eva.tex <==
\begin{table}[t]
\caption{Automatic evaluation results of the generated documents. 
``pipeline'' refers to generated documents processed by the full three-stage pipeline, and ``direct rephrasing'' refers to generated documents that are directly rephrased by ChatGPT without grouping, ordering and aggregating process. 
}
\label{dataset_eva}
\centering
\scalebox{0.85}{
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Metric}} & pipeline & direct rephrasing \\ \hline
FINE-omission                         & 0.9049            & 0.8842            \\ \hline
FINE-hallucination                    & 0.9103            & 0.8838            \\ \hline
ESA-entity                            & 0.9707            & 0.9663            \\ \hline
ESA-action                            & 0.9648            & 0.9573            \\ \hline
\end{tabular}
}
\end{table}


==> tables/dataset_eva_human.tex <==
\begin{table}[]
\begin{tabular}{ccccccccccccccc}
\multirow{3}{*}{method} & \multicolumn{4}{c}{Automated Evaluation}            & \multicolumn{10}{c}{Human Evaluation}                                                                                                                                 \\
                        & \multicolumn{2}{c}{FINE} & \multicolumn{2}{c}{ESA}  & \multicolumn{2}{c}{Understandable} & \multicolumn{2}{c}{Adequacy} & \multicolumn{2}{c}{Hallucination} & \multicolumn{2}{c}{Coherence} & \multicolumn{2}{c}{Humanness} \\
                        & omission & hallucination & omission & hallucination & score            & ICC             & score         & ICC          & score            & ICC            & score          & ICC          & score          & ICC          \\
DT                      & -        & -             & -        & -             & 4.13             & 0.91            & 4.15          & 0.92         & 4.41             & 0.92           & 3.25           & 0.9          & 3.11           & 0.92         \\
DT+chatgpt              & 0.8842   & 0.8838        & 0.9663   & 0.9573        & 4.45             & 0.9             & 4.48          & 0.92         & 4.48             & 0.89           & 4.4            & 0.89         & 4.37           & 0.93         \\
ours                    & 0.9049   & 0.9103        & 0.9707   & 0.9648        & 4.51             & 0.93            & 4.57          & 0.94         & 4.59             & 0.92           & 4.49           & 0.9          & 4.43           & 0.92        
\end{tabular}
\end{table}

==> tables/dataset_human.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Human evaluation results of the generated procedural documents.
}
\label{dataset_human}
\centering
\scalebox{0.75}{
\begin{tabular}{|l|cc|cc|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Criterion}}} & \multicolumn{2}{c|}{pipeline}     & \multicolumn{2}{c|}{direct rephrasing} & \multicolumn{2}{c|}{direct concatenating} \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                    & \multicolumn{1}{c|}{Score} & ICC  & \multicolumn{1}{c|}{Score}    & ICC    & \multicolumn{1}{c|}{Score}     & ICC      \\ \hline
Understandable                                            & \multicolumn{1}{c|}{4.51}  & 0.93 & \multicolumn{1}{c|}{4.33}     & 0.89   & \multicolumn{1}{c|}{3.59}      & 0.92     \\ \hline
Adequacy                                                  & \multicolumn{1}{c|}{4.57}  & 0.94 & \multicolumn{1}{c|}{4.37}     & 0.91   & \multicolumn{1}{c|}{4.02}      & 0.89     \\ \hline
Hallucination                                             & \multicolumn{1}{c|}{4.59}  & 0.92 & \multicolumn{1}{c|}{4.47}     & 0.89   & \multicolumn{1}{c|}{4.11}      & 0.93     \\ \hline
Coherence                                                 & \multicolumn{1}{c|}{4.49}  & 0.90 & \multicolumn{1}{c|}{4.05}     & 0.90   & \multicolumn{1}{c|}{3.17}      & 0.89     \\ \hline
Humanness                                                 & \multicolumn{1}{c|}{4.43}  & 0.92 & \multicolumn{1}{c|}{4.31}     & 0.92   & \multicolumn{1}{c|}{2.86}      & 0.90     \\ \hline
\end{tabular}
}
\end{table}

==> tables/improvement.tex <==
\begin{table}[]
\caption{Results of proposed framework and corresponding baseline models. Best results are represented in bold.
}
\label{tab:improve}
\centering
\scalebox{0.9}{
\begin{tabular}{|l|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Model}} & \textbf{XOR}    & \textbf{OR}     & \textbf{AND}    \\ \hline
ChatGPT                              & 0.4459          & 0.0672          & 0.1284          \\ \hline
Llama2 fine-tuned                    & 0.5539          & 0.0900          & 0.3979          \\ \hline
self-refined ChatGPT                 & 0.5085          & 0.2487          & 0.4081          \\ \hline
self-refined Llama2                 & \textbf{0.5814} & \textbf{0.2983} & \textbf{0.4511} \\ \hline
\end{tabular}
\vspace{-0.3cm}
}
\end{table}


